#PoetsOfInstagram: Navigating The Practices And Challenges Of Novice Poets On Instagram

Commencing as a photo-sharing platform, Instagram has since become multifaceted, accommodating diverse art forms, with poetry emerging as a prominent one. However, the academic understanding of Instagram's poetry community is limited, yet its significance emerges from its distinctive utilization of a primarily visual social media platform guided by recommendation algorithms for disseminating poetry, further characterized by a predominantly novice creative population. We employ qualitative analysis to explore motivations, experiences, and algorithmic influence within Instagram's poetry community. We demonstrate that participants prioritize conforming to algorithmic constraints for visibility, yet maintain their community's values of integrity and originality, illustrating the tension between algorithmic growth and participant authenticity. We introduce the concept of Algorithmically Mediated Creative Labor, a phenomenon specific to non-monetizing creative users who are impacted by the prioritization of professional creators and continually adapt their creative endeavors to align with platform logic, thereby affecting their motivation and creative outputs.

==> FutureWork.tex <==

Beginning with data, collection methods can include API collection, or content analysis using certain hashtags to perform an observatory study of the themes and lengths of poetry posted.  Prior studies have proven various findings about communities of practice on Instagram \cite{articlecop, barta} the community can further be inspected and their practices, as a collective group can be reduced into thematic categories, to infer ways in which the algorithm impacts the practices. Moreover, bigger and longer experiments can be conducted to manipulate and study the actual workings of the algorithm. For instance, as an independent variable, a certain profile's interactions can be guided and manipulated, and researchers can observe the behaviour of the algorithm, and the impact it has on the performance of the particular profile. Furthermore, an interview of participants who have a bigger number of followers could be conducted, wherein an interesting cross amidst influential poets, who identify themselves as the faces of the poetry community. More studies in terms of difference in content between digitally published poetry on social media and poetry published in hard copies can be further studied\cite{articlecomp}. Finally, as this study intends to work on providing poets with more efficient sharing and collaboration, review of the problems and motivations of poets writing in other languages can also be compared, to gather data and create an independent platform specific to poetry sharing.  
